Online structural kernel selection for mobile health

Motivated by the need for efficient and personalized learning in mobile health, we investigate the problem of online kernel selection for Gaussian Process regression in the multi-task setting. We propose a novel generative process on the kernel composition for this purpose. Our method demonstrates that trajectories of kernel evolutions can be transferred between users to improve learning and that the kernels themselves are meaningful for an mHealth prediction goal.

==> icml workshop/overflow.tex <==
Here is what I think this model is saying: 
\begin{enumerate}
    \item Previously, the Dirichlet process encoded the clusters of kernel compositions across users
    \item Now, there is a separate DP for every non-leaf node in the tree. For the a given node ($A$), the DP now represents the \textbf{different possible branches (caused by different users)} from ($A$). For example, we have already observed many users going from ($\mathrm{LIN}) \rightarrow (\mathrm{LIN + PER}$) composition. Then we start observing a bunch of users go from $(\mathrm{LIN}) \rightarrow (\mathrm{LIN + SE})$ composition. The $DP(\alpha, H_0 | \mathrm{LIN})$ allows us to capture this as "two separate clusters leaving from $\mathrm{LIN}$"
    \item This means the overall trajectory tree is built by letting each DP grow its branches. Essentially every time a node "branches" (i.e the DP at that node finds a new cluster), it adds another DP to the model. Should DPs that are further down the tree (i.e. the parent node represents a more complex composition) have stricter concentration parameters? Basically, should we make it harder for more complex compositions to branch even further? 
    \item \sam{I am unsure about  the level at which we are clustering.  It seems like we should cluster users (e.g. a cluster has common kernel for their ground truth reward function).  Then when a new user arrives the new user would from the DP have cluster membership probabilities-- a probability to join each existing cluster and a probability to form a new cluster (probabilities sum to 1).  After x time points for this user (data-- this user's (S,A,R) for x time points), the cluster membership  probabilities for this user would be updated. The bias-variance tradeoff would occur when the new user, initially has a higher probability of being in a cluster with a simple kernel, like LIN but then as data on this new user accrues the posterior cluster membership probabilities may change to a more complex kernel such as LIN +PER.   }
\end{enumerate}

Susan made a really interesting point that \emph{rate at which a user traverses the tree} is dependent on their noise level, $\sigma_n^2$. For example, consider the trajectory $(\mathrm{""}) \rightarrow (\mathrm{LIN}) \rightarrow (\mathrm{LIN + PER})$. 
\begin{itemize}
    \item If the timestep represents $20$ new data points, user $1$ may traverse the tree normally $(\mathrm{""}) \rightarrow (\mathrm{LIN}) \rightarrow (\mathrm{LIN + PER})$.
    \item But user $2$ may have VERY noisy rewards. So he/she may need a relatively higher number of points before realizing a more complex function. The trajectory for user $2$ could look something like $(\mathrm{""}) \rightarrow (\mathrm{LIN}) \rightarrow (\mathrm{LIN}) \rightarrow (\mathrm{LIN}) \rightarrow (\mathrm{LIN + PER})$
    \item Finally, user $3$ could have very little noise and jump almost instantaneously to the last node:$(\mathrm{""}) \rightarrow (\mathrm{LIN + PER})$
\end{itemize} 

I don't think this should affect how we represent/train the model? It may mean that each node should/will likely find a self-loop (to accomodate the noisy).


Below is work in progress and likely not correct
\begin{algorithm}[H]
\label{alg: inference blocked gibbs sampling}
  \SetAlgoLined
  \SetKwInOut{Input}{input}
  \SetKwInOut{Output}{output}
  \Inp{Data for $M$ tasks with $T_m$ time steps per task, max number of clusters $N$ in truncated stick-breaking representation}
  \SetKwProg{Initialize}{Initialize.}{}{}
  \Initialize{} {
  The set of parent clusters, $\mathbf{K} = \{K_0\}$\;
  }
  
  \SetKwProg{ClusterUpdate}{Update clusters.}{}{}
  \ClusterUpdate{} {
    \For{$K \mathrm{\ in\ } \mathbf{K}$} {
      Optimize for kernel hyperparameters $\boldsymbol{\theta}$: \; \\
        $\mathbf{X}_K = \left \{\mathbf{X}_{m, t-1} | K_{m, t-1} = K \right \}$ \;\\
        $\mathbf{y}_K = \left \{\mathbf{y}_{m, t-1} | K_{m, t-1} = K  \right \}$ \;\\
        Find MAP estimate of $\boldsymbol{\theta}$ by optimizing $p(\mathbf{y}_K | X_K, \boldsymbol{\theta})p(\boldsymbol{\theta} | K)$ \; \\
        
      \For{c = 1, \ldots, N} {
        Update cluster membership probabilities: \; \\
            $V^{(K)}_c \sim \mathrm{Beta}\left (1 + n_c^{(k)}, \alpha + \sum\limits_{c' = c + 1}^{N} n_{c'}^{(K)} \right)$ \; \\
            $\pi^{(K)}_c = V^{(K)}_c \prod\limits_{\ell < c}(1 - V_\ell)$  \; \\
            
        Update kernel distribution at each cluster: \; \\    
        \If{n_c^{(K)} = 0}{
            $\eta^{(K)}_c \sim H_0$
        }
        \Else{
            How to update $\eta$???
        }
      }
    }
  }

  \SetKwProg{ClusterAssignment}{Assign tasks to clusters.}{}{}
  \ClusterAssignment{} {
    \For{m = 1, \ldots, M}{
      K_{m, 0} = K_0 \; 
      
      \For{t = 1, \ldots, T_M}{
        K = K_{m, t - 1} \; \\
        \For{c = 1, \ldots, N}{
          p(Z_{m, t} = c) = \frac{\pi_c^{(K)} p(\mathbf{y}_{m, t} | \eta^{(k)}_c)}{\sum\limit_{c' = 1}^N \pi_{c'}^{(K)} p(\mathbf{y}_{m, t})} \; \\
        }
      }
    }
  }
 $\mathbf{K}$ = unique kernels  
\caption{Block Gibbs Sampling for Kernel Trajectories}
\end{algorithm}


\section{Introduction}
In this paper we develop a generative process of compositional kernel learning for the online, multi-task setting. The choice of kernel is critical to the performance of a Gaussian Process (GP) regression model, and the best kernel is often \emph{task and data dependent}. Compositional and/or structural kernels themselves offer many benefits over the popular SE ARD kernel. Compositional kernels are interpretable \cite{schulz2016probing, lloyd2014ABC}, have better generalization in the presence of global structure \cite{duvenaud2011additive, duvenaud2013cks, steinruecken2019automaticStatistician}, and have been used to improve Bayesian Optimization \cite{gardner2017hmcBayesOpt, sun2018differentiable}.

A promising yet unexplored application of compositional kernels is the online data setting. Here, we can add or remove kernel components as a way to increase or decrease the complexity of our model. Intuitively this means the model's representation power can grow as the data, and its observable structures, also grows. The multi-task learning (MTL) scenario is a natural counterpart to the online setting. In many practical applications, one must solve multiple problems in tandem but may wish to exploit the shared information among the related tasks. 

One such example is mobile health (mHealth), which motivates our work in this area. This is a sequential decision making problem, where the goal is to maximize the patient's healthy behaviors through a series of personalized interventions. For example, Heartsteps is a fitness app where the goal is to maximize the patient's step count (behavior) following a push notification (intervention). The learning algorithm is able to observe data from all users on the app as it arrives, but must personalize the interventions to each patient. 
%this could be deleted 
mHealth is a particularly challenging environment for learning because the task-level data is sparse, noisy, and high dimensional. 

Structural kernel search is already a difficult and open research problem with batch data; deploying existing methods online will exacerbate current challenges and create new ones. Unlike with batch data, streaming data means we have to reconsider the entire composition as new data arrives. Discrete kernel search methods \cite{ duvenaud2013cks, kim2018scaling, sun2018differentiable} are not suitable because you would have to restart the entire search process from scratch to readjust the kernel to any new data. 
% FDV: Be careful with statements like the above: a reader could say, "Why not wait and update in batches?" -> express the core issue about repeatedly starting from scratch (which is real) in a way that can't be argued.
Probablistic methods \cite{gardner2017hmcBayesOpt, titsias2011spike, tong2020shrinkage} are naturally suited to this task because Baye's rule allows the previous compositional posterior to form the new prior. 

% Expand on this in the model selection background
Kernel search is also a layered problem which requires one to select the kernel (model) and then the hyperparameters. Current methods overwhelmingly rely on some form of ML-II optimization \cite{mackay1999comparison, books/lib/RasmussenW06} to approximate the model evidence. These approaches are sensitive to local optima and require multiple random restarts \cite{duvenaud2013cks, kim2018scaling} or duplicitous kernels \cite{tong2020shrinkage, sun2018differentiable} for correct model comparison.  Furthermore, optimization in this setting is computationally expensive due to the kernel inversions required for calculating the GP marginal likelihood. 

The above search and optimization challenges would clearly benefit from some form of transferred knowledge, which could better inform the model prior and warm start the optimization. In this paper, we develop a generative process to capture how kernel compositions evolve with growing data. Furthermore, we explore the idea that these trajectories of kernel evolution can be \emph{transferred} between tasks. 
We demonstrate that (\textbf{will update based on model}): 
\begin{itemize}
    \itemsep 0.1em
    \item Our model can leverage past data from other kernel trajectories to better understand how a new tasks's kernel is likely to evolve
    \item Learning group-level kernel trajectories has comporable performance to the completely task-level baselines, while improving speed and interpretability
    \item We demonstrate the effectiveness of our approach on a real world application in mobile health 
\end{itemize}

